Incentivizing Truthfulness Through Audits in Strategic Classification

In many societal resource allocation domains, machine learning methods are increasingly used to either score or rank agents in order to decide which ones should receive either resources (e.g., homeless services) or scrutiny (e.g., child welfare investigations) from social services agencies. An agency's scoring function typically operates on a feature vector that contains a combination of self-reported features and information available to the agency about individuals or households.This can create incentives for agents to misrepresent their self-reported features in order to receive resources or avoid scrutiny, but agencies may be able to selectively audit agents to verify the veracity of their reports. We study the problem of optimal auditing of agents in such settings. When decisions are made using a threshold on an agent's score, the optimal audit policy has a surprisingly simple structure, uniformly auditing all agents who could benefit from lying. While this policy can, in general, be hard to compute because of the difficulty of identifying the set of agents who could benefit from lying given a complete set of reported types, we also present necessary and sufficient conditions under which it is tractable. We show that the scarce resource setting is more difficult, and exhibit an approximately optimal audit policy in this case. In addition, we show that in either setting verifying whether it is possible to incentivize exact truthfulness is hard even to approximate. However, we also exhibit sufficient conditions for solving this problem optimally, and for obtaining good approximations.

==> Approximations.tex <==
\section{Approximations}

\subsection{Threshold}



    
    \subsection{Top-$k$}
    
    
    
    
\subsection{Exact Solutions for Large $n$ and discrete $D$}

\textcolor{blue}{Since we are adding results for large $n$, perhaps it makes sense to discuss the fact that in certain settings large enough $n$ makes the problem trivially tractable}

The aforementioned approximation algorithms improve in both their tightness of approximation, and probability of success as $n$ increases.
For \emph{large} $n$ these algorithms produce approximations that are very close to actual solutions. 
However, it is worth mentioning that in several settings where $n$ is \emph{large}, exact solutions can be computed in polynomial time for discrete $D$. More specifically, when the size of the attribute vector is dominated by the number of agents, the problem becomes tractable.
This is simply by virtue of the fact that computation of the cumulative joint distribution is trivially in polynomial time.

\begin{theorem}
    Suppose that $D$ is discrete and $|I| \in \Theta(1)$. If $n$ is sufficiently large, $n >> s + d$, such that $s + d \leq \Theta(\log(n))$, then computing minimum $\epsilon$BNIC in both threshold and top-$k$ allocation can be done in polynomial time.
\end{theorem}

\begin{proof}
    Since $s + d\leq \Theta(\log(n))$, computing the value of $f(\x, \z)$ for all possible agent types can be done in time $\Theta)(|I|^{s + d}) = \Theta(|I|^{\log(n)}) = \Theta(n)$.
    As a byproduct, computing the partitions $U_{\theta} = \{(\x, \z) \in \inter: f(\x, \z) \geq \theta \}$ and $L_{\theta} = \{(\x, \z) \in \inter: f(\x, \z) < \theta \}$ are trivially in polynomial time. Moreover, computing the probability that an agent falls into either partition is also computable in time $\Theta(n)$. With both these values computed, the rest of the problem follows in polynomial time. 
\end{proof}


    
    
    
    
    
    
    


==> Case_Study.tex <==

\section{Case Study}

Suppose the objective of the principal is, given a score function, produce an audit policy such that truthful reporting of $\z$ is an equilibrium. Consider the following example $\alpha = \beta = 1$ (i.e. one known, and one self-reported, attribute) and $f(\x, \z) = x + z$. Denote the common prior  $\mathbb{P}\big(\aj_i = (x, z)\big) = p_{x, z}$,the number of agents the principal intends to audit from each group as $\theta_{x, z}$, and the random variable representing the population size of type $(x, z)$ as $N_{x, z}$.


Note that only agents of type $(1, 0)$ and $(0, 0)$ have motive to report false $z$. Therefore $\theta_{1, 0} = \theta_{0, 0} = 0$. 
Let $t_{1, 0}, t_{0, 0}$ be the expected value of an agent of either type truthfully reporting $z$ and $l_{1, 0}, l_{0, 0}$ be the expected value of an agent falsely reporting $z$.

The principals objective is then to determine if there is a satisfying assignment to $\theta_{1, 1}, \theta_{0, 1}$ such that
\begin{align*}
    t_{1, 0} \geq l_{1, 0}
    t_{0, 0} \geq l_{0, 0}
    \theta_{1, 1} + \theta_{0, 1} = B
\end{align*}


Let $\aj_i = (1, 0)$. If all other agents are truthful, then the expected value of $\aj_i$ reporting $z' = 0$ is 
\begin{align}\label{10tru}
    t_{1, 0} = \mathbb{P}\big(N_{1, 1} + N_{1, 0} \geq k) + \mathbb{E}\bigg[ \frac{k - N_{1, 1}}{N_{1, 0}}\bigg]\bigg|_{N_{1, 1} < k < N_{1, 1} + N_{1, 0}}
\end{align}
and the value for reporting $z' = 1$ is 
\begin{align}\label{10lie}
    l_{1, 0} = \mathbb{E}\bigg[ \max\bigg(0, 1 - \frac{_{1, 1}}{N_{1, 1} + 1}\bigg)\bigg]\bigg|_{k \geq N_{1 , 1} + 1} + \mathbb{E}\bigg[\max\bigg(0, 1 - \frac{\theta_{1, 1}}{N_{1, 1} + 1}\bigg) \frac{k}{N_{1, 1} + 1}\bigg]\bigg|_{N_{1, 1} + 1 > k}
\end{align}

For any given $k$ Expression \ref{10tru} is independent of $\theta_{1, 1}$ and  $\theta_{0, 1}$, and we can express Expression \ref{10lie} as
\begin{align} 
      l_{0, 1} = &\sum_{i = \theta - 1}^{k - 1} \bigg(1 - \frac{\theta_{1, 1}}{i + 1}\bigg)p_{1, 1}^i (1 - p_{1, 1})^{n - i} \binom{n}{i} + \sum_{i = \max(k - 1, \theta_{1, 1} - 1)}^n\frac{k}{i  + 1} \bigg( 1 - \frac{\theta_{1, 1}}{i + 1}\bigg)
    %=&-\theta_{1, 1}\sum_{i = \theta - 1}^{k - 1}\bigg(\frac{1}{i + 1}\bigg)p_{1, 1}^i (1 - p_{1, 1})^{n - i} \binom{n}{i} + \sum_{i = \theta - 1}^{k - 1} p_{1, 1}^i (1 - p_{1, 1})^{n - i} \binom{n}{i}
\end{align}
Similarly expressions for an agent of type $(0, 0)$ truthfully reporting $z$ as

\begin{align}\label{tru00}
    t_{0, 0} = \mathbb{E}\bigg[ \frac{k - N_{1, 1} - N_{1, 0} - N_{0, 1}}{N_{0, 0}} \bigg]\bigg|_{k > N_{1, 1} + N_{1, 0} + N_{0, 1}}
\end{align}
and the expect value of agent for falsely reporting $z$ as,
\begin{align}\label{lie00}
     l_{0, 0} = &\mathbb{E}\bigg[ \frac{k - N_{1, 1} - N_{1, 0}}{N_{0, 1} + 1}\max\bigg(0, 1 - \frac{B - \theta_{1, 1}}{N_{0, 1} + 1}\bigg)\bigg] \bigg|_{N_{1, 1} + N_{1, 0} + N_{0, 1} >  k \geq N_{1, 1} + N_{1, 0}}\\
    +&\mathbb{E}\bigg[\max\bigg(0, 1 - \frac{B - \theta_{1, 1}}{N_{0, 1} + 1}\bigg) \bigg]\bigg|_{k\geq N_{1, 1} + N_{1, 0} + N_{0, 1}}
\end{align}
As in the case of agents of type $(1, 1)$ we see that Expression \ref{tru00} is independent of $\theta_{1, 1}$. Further, note that Expression \ref{lie00} can be expressed as a sum of at most $n$ terms in similar fashion to expression \ref{10lie}. 

Since we can express each $l_{x, z}$ as an expression which is monotone in $\theta_{1, 1}$ and $\theta_{1, 1}$ takes on at most $B$ values, we can binary search over the space of $\theta_{1, 1} \in [B]$ to find if there exists a $\theta_{1, 1}$ that satisfies both constraints. 

==> Ex1.tex <==
%%%%%%%%%%%%%%%%%%%%%
\begin{example}\normalfont 
    Suppose there are $n = 2$ agents with attributes of the form $(x, z) \in \{0, 1\} \times \{-1, 0, 1\} $. Suppose the common prior on agent types is given by a distribution $D$ with PMF.
    \begin{align*}
        h(x, z) = 
        \begin{cases}
        \beta &\text{ if } $z = 1$ \\
        \frac{1 - 2\beta}{4} &\text{ otherwise} 
        \end{cases}
    \end{align*}

    Suppose the score function is given by $f(x, z) = x + 2z$ with threshold $c = 0$.
    
    First observe that only agents of type $(0, -1)$ and $(1, -1)$ have incentive to deviate from truthful reporting. Both types of agents have sufficiently high scores for a resource when reporting $\eta(z) \in \{0, 1\}$. Let $r = 1$ and $C = 3$.
    
     Suppose that $\aj_1 \in \{ (0, -1), (1, -1) \}$. Under UNIFORM, if $\aj_1$ submits either $\eta_1(z_1) = 0$ or $\eta_1(z_1) = 1$, then the probability that $\aj_1$ is selected for audit is 
     \begin{align*}
        \phi_{(x', z')}  = \frac{1}{2}\bigg( 2\beta + \frac{1 - 2\beta}{2} \bigg) = \frac{1 + 2 \beta}{4} \quad \text{ for } x', z' \in \{0, 1\}
     \end{align*}
    
    Then the expected difference in $\aj_1$'s utility, when submitting either lie is
    \begin{align*}
        v_1 = \mathbb{E}[\aj_1 \text{ lying}] = \big(1 - \phi_{(x', z')}\big)  - \phi_{(x', z')} = 1 - 4 \frac{1 + 2\beta}{4} = 1 - (1 + 2\beta) = \frac{1}{2} - \beta 
    \end{align*}
    
    For vanishing small $\beta$, agents of types $(0, 1)$ and $(1, 1)$ become increasingly unlikely and as such, the principal is increasingly suspicious of any agent submitting either value. 
    Suppose the principal has an alternative audit policy $\theta$ which accounts for the suspiciousness of reports.
    Consider the choice of auditing when an agent reports $(1, 1)$. Since $\theta$ is biased towards suspicious reports, $\theta_{(1, 1)} = \phi_{(1, 1)} + \Delta_{(1, 1)}$ for some $\Delta_{(1, 1)} > 0$. Since $\sum_{x, z = 0}^1\theta_{(x, z)} = 1$, for some $(x', z') \in \{(0, 0), (0, 1), (1, 0)\}$ it must be the case that $\theta_{(x', z')} = \phi_{(x', z')} - \Delta_{(x', z')}$ where $\Delta_{(x', z')} > 0$.
    Under this audit policy, consider the case when $\aj_1 = (x', -1)$. The expected value of $\aj_1$ submitting $\eta_1(-1) = z'$ is
    \begin{align*}
        \mathbb{E}[\aj_1 \text{ lying}] = 1 - 2\theta_{(x', z')} = 1 - 2\big(\phi_{(x', z')} - \Delta_{(x', z')} \big) = \frac{1}{2} - \beta + 2 \Delta > \frac{1}{2} - \beta = v_1
    \end{align*}
    Therefore, if the principal attempts to bias the audit policy to more suspicious reports of $(0, 1), (1, 1)$, then an agent of either type $(0, -1), (1, -1)$ will have a greater incentive to lie.
\end{example}
%%%%%%%%%%%%%%%%%%%


==> Impact.tex <==

\section{Broader Impact}
Algorithmic decision making plays an increasingly important role in high-stakes resource allocation settings, including school acceptance, loan applications, housing for the homeless, and welfare. 
%Decisions made in these settings have significant impact on the lives of those depending on their decision making ability. 
%Common examples of these systems include welfare, school acceptance, loan applications, and many more.  
%Welfare is of particular consideration as it is an example in which proper decision making can be paramount to the lives of those who depend on the system’s support.
In such resource allocation problems, decisions are often made based on collecting individual attributes that are subsequently used as features input to a scoring function, and resource allocation decisions are then made favoring those with higher or lower scores (depending on context).
However, while some of these attributes are directly known to the decision maker, many are often self-reported, for example, through surveys.
As a result, individuals may often have an incentive to misreport their self-reported characteristics in order to increase the odds of receiving favorable treatment, potentially resulting in  inefficient and inequitable decisions.
Consequently, an important concern for policy makers is to ensure that attributes ascribed to individuals accurately represent them, which entails reducing incentives to misreport self-reported features.

%agents can often strategically alter the value of particular attributes that are used in the decision process. 
%Naturally, this leads to the potential for agents to dishonestly represent themselves with the hopes of obtaining a resource. 
%These resources are often scare, meaning that dishonest agents could deprive agents actually in need, of a resource. 
%Our work aims to protect such systems and ensure that it is in an agents best interest to truthful report their attributes. 

We study the problem of auditing individuals based on their reported attributes, a common tool in policy making to incentivize truthful reporting (e.g., IRS audits).
Our investigation centers around two questions: computational verification of whether incentives to misreport preferences exist (and how strong they are), and characterization of audit policies that minimize such incentives.
Both have practical significance: the first in enabling assessment about how concerned we should be about incentives in particular settings, and the second in prescribing the best ways to reduce the incentives to game the system.

Our approach has several limitations.
First, our model assumes that individuals do not incur any direct cost from misreporting preferences.
In reality, misreporting may be costly, both cognitively and in more tangible ways, such as effort it takes to identify the most valuable lie.
Second, we do not explicitly consider inadvertent errors.
While in principle audits as they are implement can attempt to distinguish between deliberate and accidental lies, this is unlikely to be perfect, potentially resulting in unfair punishments.
Third, we assume that the distribution over agent types is known a priori.
While a common assumption in game theory and mechanism design, it is unlikely to hold in practice.
Rather, we will need to estimate this distribution from past experience in particular resource allocation settings.

In terms of potential use of our ideas in practice in the future, one positive aspect is that uniform auditing turns out to be optimal for indicuing BNIC equilibria in the threshold setting. The simplicity of a uniform lottery makes it easy to explain and is likely to also make it widely acceptable in public perception. In the top-k setting, if more complex but better auditing mechanisms are found, they may not be as easy to get public buy-in (and understanding) for. In any case, we urge careful collaboration with stakeholders in any future deployments informed by the research in this paper. 

%Truthful incentivisation is done by auditing a subset of agents. 
%If an agent is found to have misreported their attributes, they lose the ability to obtain a resource and also pay a fine. 
%Our work designs these policies such that agents reporting truthfully constitutes an equilibrium strategy. 
%The positive side of these audit policies is that they help to ensure that honest agents are not negatively impacted by dishonest agents and thus vulnerable members of the population do not have to suffer the consequences of manipulation.
%On the other hand, our model fails to differentiate between intentional dishonesty and unintentional dishonesty. 
%As a result, a person who should qualify for welfare may make an accidental misreport on their application. 
%If caught by an audit, this person would be both denied welfare and made to pay a fine. 
%Such cases are undesirable as we wish only to dissuade intentionally dishonest agents and not to punish agents who accidentally make benign misreports, but are in need of assistance.  
%Moreover, these audit policies may force vulnerable members of the population to inherit risk by lying in instances where their chance of resource allocation is low.
%The audit policy may not guarantee that truthful reporting is an equilibrium strategy, or even a unique equilibrium strategy. 
%As such, an agent may qualify for allocation when all agents report truthfully, but under another equilibrium strategy that agent would have to misreport in-order to obtain a resource.
%Without auditing these agents do not inherit risk because there is no penalty for lying, however once auditing is introduced these agents must decide between two undesirable outcomes, being caught lying, or potentially not receiving needed assistance.
%Our aim is to minimize the negative impact to agents by reducing the amount these systems can be gamed. 
%Realizing this goal through auditing will help distribute resource to those who need them, however several potentially negative side affects can arise from the way in which agents are treated when found to have misreported.

==> Infinite_Agents.tex <==
\section{Infinite Agents}

The interactions between agents and the principal can modeled as a non-atomic game. When examined from this perspective, agents can be thought of as existing in a continuum, which can be superimposed onto the interval $[0, 1]$. When the number of agents is infinite, any individual agent is infinitely ``small", in the sense that the actions of any particular agent will have no effect on the equilibrium behavior of other agents.

To account for the infinite number of agents, the principal will audit some $B\in (0, 1)$ fraction of agents. 
Under top-$k$ allocation for infinite agents, the top $k\in (0, 1)$ fraction of agents are allocated a resource. 

The problem is fundamentally unchanged when resources are distributed according to a threshold and UNIFORM is still the optimal audit policy. 
In the case of top-$k$ allocation, we will show that the problem reduces down to an instance of threshold allocation and as such UNIFORM, for a particular threshold value, is the optimal audit policy.  
In general computing the value of this threshold will be hard from the agents perspective. 
However the principal can easily deploy this audit strategy by simple auditing with uniform probability the top-$k$-fraction of agents. 
Additionally, this strategy of uniformly auditing the top-$k$ scoring agents will provide an efficient means with which to approximate the optimal audit policy, which improves in quality as $n$ trends towards infinity. 
Although the policy will be able to be efficiently implemented and we know it converges to optimal,  actual value of this approximation will be in general NP-hard to compute, by Theorem \ref{thm:approx_hard}.

%\subsection{Threshold}
%When resources are allocated via threshold, the fundamental problem is unchanged and we will see that again, UNIFORM yields the lowest incentive to deviate from truthful reporting, compared to any other audit policy. From the principals perspective, determining if any particular agent will perform such a deviation is done in almost an identical manner. 

%\begin{theorem}
%    For an infinite share of agents, UNIFORM is an optimal audit policy.
%\end{theorem}

%\begin{proof}
%    In the case of finite agents, the audit probability, $\phi_{(\x, \z)}$, gives the probability that an agent reporting $(\x, \z)$ will be audited. In the case of infinite agents, $\phi_{(\x, \z)}$ can be thought of as a choice to audit $\phi_{(\x, \z)}$ fraction of the agents reporting $(\x, \z)$, where the particular agents from this selected population are chosen uniformly at random. All selection methods from a population reporting the same value, $(\x, \z)$ are equivalent. Under this formulation of $\phi_{(\x, \z)}$, the proof follows directly from that of Theorem \ref{thm:bayes_nash_best_policy}. 
%\end{proof}


\begin{theorem}
    Let $T$ be the set of the top-$k$ scoring fraction of agents under truthful reporting. Let $\alpha = \min \{f(\x, \z): (\x, \z) \in T\}$. Then setting $C = \alpha$ and using UNIFORM yields the lowest value of $\epsilon$ under-which truthful reporting is an $\epsilon$-Bayes-Nash equilibrium.
\end{theorem}

\begin{proof}
    Suppose all agents truthfully report $\z$. Under this profile, we are interested in the maximum utility that any agent can gain from deviating to any lie. 
    First note that if a single agent deviates, the value of $\alpha$ is unchanged.
    Second, any optimal audit policy will never audit an agent reporting a score of $f(\aj_i) < \alpha$ since agents with these scores will not be allocated a resource. 
    Let 
    \begin{align*}
        G = \{ (\x, \z) \in \inter: f(\x, \z) \geq \alpha \land \exists \z'\in I^z \text{ s.t. } f(\x, \z') < \alpha\}.
    \end{align*}
    That is, $G$ is the set of all possible agents who could be lying. 
    Under UNIFORM, the probability of any agent $\aj_i = (\x_i , \z_i) \in G$ being audited is
    \begin{align*}
        \phi_{(\x_i, \z_i)} = B \bigg(\int_G  h(\x, \z) d\x d\z \bigg)^{-1}
    \end{align*}
    Therefore the expected value of lying can be expressed as 
    \begin{align*}
        \mathbb{E}[\text{lying}] = r\big(1 - \phi_{(\x_i, \z_i)}) - c \phi_{(\x_i, \z_i)}
    \end{align*}
    Once we have the expected value of lying in this form, we see that an agent's decision to submit any lie is equivalent to their decision to submit the exact same lie in the case of threshold allocation when the threshold is $c = \alpha$. 
    From here, the proof follows identically from the proof of Theorem \ref{thm:bayes_nash_best_policy}.
\end{proof}

Next we examine the rate of convergence of the difference between an agents expected value of lying under WGHTAUDIT and uniformly auditing the top-$k$ scoring agents. 
\begin{theorem}
    \textcolor{blue}{The bounds on approximation need work. At this point it appears the bounds are going to depends heavily on the relationship between the distribution and the score function which are currently proving to be quite unweildy in the general case.}
\end{theorem}

\begin{proof}
    Let $\phi$ denote WGHTAUDIT and $\theta$ denote uniformly auditing the top-$k$ scoring agents. Then the difference in expected values of submitting any particular lie for an agent of type $(\x_i, \z_i)$ is
    \begin{align*}
          & \mathbb{P}\big((\x_i, \eta_i(\z_i)) \in T\big)\big(\phi_{(\x_i, \eta_i(\z_i))} - \theta_{(\x_i, \eta_i(z_i)}\big)\\
        = & \mathbb{P}\big((\x_i, \eta_i(\z_i)) \in T\big)\bigg(\min\big(1, \frac{B}{k}\big)\bigg(1 - \bigg(\frac{\mathbb{P}\big((\x_i, \z_i') \in T\big)}{\mathbb{P}\big((\x_i, \eta_i(\z_i))\in T\big)}\bigg)\bigg) - \min\big(1, \frac{B}{k}\big)\mathbb{P}\big((\x_i, \eta_i(\z_i)) \in T\big)\bigg)\\
        = & \min\big(1, \frac{B}{k}\big)\bigg(1 - \mathbb{P}\big((\x_i, \eta_i(\z_i)) \in T\big)^2 - \mathbb{P}\big((\x_i, \z_i') \in T\big) \bigg)\\
    \end{align*}
\end{proof}

==> RelatedWork.tex <==
\section{Related Work}

\textcolor{blue}{Still need to complete}

==> dsic.tex <==
In similar fashion, finding the ``best" audit policy, when the goal is to make truthful reporting a dominant strategy, is straightforward, but determining if that policy causes the threshold allocation mechanism to be \dominant is \#P-hard.
We again use the term ``best" to indicate that the policy induces an $\epsilon-$equilibrium for the minimum value of $\epsilon$.

\begin{theorem}\label{thm:best_dominant}
       For any score function $f$, any distribution $D$ with nonzero support, UNIFORM induces truthful reporting to be an $\epsilon$DSEQ for the smallest possible value of $\epsilon$ under any audit policy.
\end{theorem}

\begin{proof}
As shown previously, under the threshold allocation, if agents value the resource at $r$ and incur cost $c$ when caught lying, then the expected utility of lying is 
\begin{align*}
    r(1 - \phi) - \phi c
\end{align*}
where $\phi$ is the probability the lying agent is audited. 
Therefore, lying has an expected positive utility only when $\phi < \frac{r}{r + c}$.

When examining the Bayes-Nash equilibrium, each $\phi$ depended only on the underlying distribution, i.e. $\phi$ was determined by the expected number of agents who would be truthfully reporting $(\x, \z)$ such that $f(\x, \z) \geq 0$. In this case $\phi$ is now a function of the choices of other agents since the probability of being audited under UNIFORM is uniquely determined by the number of agents with positive score, truthful or otherwise. However, a partial ordering is easily induced, on the strategy profiles of the other agents, by counting the number of agents who report $f(\x, \z) \geq 0$. Under the, up-to $2^n$, different outcomes of $g(f(\x_i, \z_i'))$ are condensed down to $n$ unique equivalence classes. Since the principal uniformly audits up to $B$ agents reporting non-negative scores,  we see that $\phi$ is monotonically decreasing as with respect to the partial ordering induced on agent action profiles. Which implies a monotonic expected value of lying, with respect to the partial ordering, i.e. we need only investigate the case when $\phi$ is minimized.
In this case, the proof is identical to that of Theorem \ref{thm:bayes_nash_best_policy}, with the exception that the set $G$ be replaced by $G \cup S$.
\end{proof}

\begin{theorem}\label{thm:domEQ}
        Under the same setting as specified in Theorem \ref{thm:nashEQ}, determining if UNIFORM can cause DSIC can be computed in polynomial time. 
\end{theorem}

\begin{proof}
Again defined the sets
 \begin{align*}
        G &= \{ (\x, \z) \in I^d \times I^s : f(\x, \z) \geq 0\}\\
         S &= \{ \aj \in I^d\times I^s: f(\x, \z) < 0 \land \exists\z'\in I^s \text{ with } (\x, \z') \in G\}
    \end{align*}
If the mechanism is to be \dominant, then it must be the case that for any agents $\aj$ truthful reporting of $\z$ has a higher expected utility than lying, under any action profile for the other $n - 1$ agents. As shown in the proof of Theorem \ref{thm:best_dominant}, the worst case for the a principal using UNIFORM, i.e. $\phi_{aj}$ is minimized for all $\aj \in A$, arises when all agents in $S$ choose to lie and all agents in $G$ are truthful. This is due to the fact that $G$ will be maximally populated under this action profile, compared to any other action profile. 
In the proof of Theorem \ref{thm:nashEQ}, our strategy was to compute the measure of $h(G)$, as this value determined the audit probability $\phi_{\aj}$. Again we have that truthful reporting is a dominant strategy if and only if $\phi_{\aj} \leq \frac{r}{c + r}$ for all $\aj\in I^d\times I^s$. 
However, we require this to be true under every action profile, which are all subsumed by principal's worst case action profile. Thus, in the current setting $\phi_{\aj}$ is now determined by $h(G \cup S)$. 
Note that $G \cup S$ is not necessarily the entire space of $I^d\times I^s$.
Let $p_{G\cup S} = \int_{G\cup S} h(\x, \z)$. 
Then, we again have that trustful reporting is a dominant strategy if and only if 
\begin{align*}
        \phi_{\aj} = \sum_{\ell = 0}^n \binom{n}{\ell} p_{G\cup S}^{\ell}(1 - p_{G\cup S})^{n - \ell} \min\bigg(1, \frac{B}{\ell}\bigg)\geq \frac{r}{r + c}
\end{align*}
Since $G\cap S = \emptyset$, we have that $\int_{G \cup S} h(\x, \z) = \int_G h(\x, \z)dG + \int_S h(\x, \z)dS$. Computing $\int_G h(\x, \z)dG$ can be done in the exact fashion as in \ref{thm:nashEQ}. To integrate over $S$ we will again use the trick of expressing $S$ as the cross product of simple intervals. In the derivation of $\int_G h(\x, \z)$, the intervals defining $G$ were given by $[x_a^*, \hat{x}_a]$, again using $x$ rather than $z$ only for ease of notation. The value of $x_a^*$ is a maximizer of $f$, and $\hat{x}_a$ either corresponded to the zero of the separating hyperplane induced by $f$, or was the value at the extreme of $I$, opposite to $x_a^*$. Note that if the latter is true, then the corresponding $a^{\text{th}}$ dimension of $S$ should be empty, otherwise the $a^{\text{th}}$ dimension of $S$ is $[x^*_a, \hat{x}_a]^c$, with respect to $I$. Therefore, $S$ may also be written as the cross product of simple intervals Fubini's Theorem may again be used to calculate $\int_S h(\x, \z) dS$. Thus yielding the value of $p_{G\cup S}$ and allowing us to immediatly determine if 
\begin{align*}
    \sum_{\ell = 0}^n \binom{n}{\ell} p_{G\cup S}^{\ell}(1 - p_{G\cup S})^{n - \ell} \min\bigg(1, \frac{B}{\ell}\bigg)\geq \frac{r}{r + c}
\end{align*}
In which case, truthful reporting is in fact a dominant strategy.

\end{proof}

\begin{corollary}\label{cor:piece_dom}
   For $f$ piecewise linear and an identical setting as Corollary \ref{cor:piecewise-nashEq}, determining if UNIFORM causes DSIC can be done in polynomial time.
\end{corollary}

\begin{proof}
This follows immediately from the proof of Theorem \ref{thm:domEQ} and Corollary \ref{cor:piecewise-nashEq}.
\end{proof}


By similar reasoning as the proof of Theorem \ref{thm:sigmoid} the following corollaries are immediate.
\begin{corollary}\label{cor:dom_sig}
   Under identical assumptions as Theorem \ref{thm:sigmoid}, determining if UNIFORM causes DSIC can be done in polynomial time for sigmoid $f$.
\end{corollary}

\begin{theorem}\label{thm:Dom_linear_top_k}
    Suppose $n$ agents are sourced from a continuous distribution $D$, with PDF $h$, over the set $I^d\times I^s$ for $I\subset \R$. Further, suppose that $h(\x, \z) > 0$ for all $(\x, \z) \in I^d \times I^s$, $f$ is linear, and resources are allocated via top-$k$. Then computing the audit policy which induces an \eDS, with the smallest $\epsilon$, and deciding DSIC, can both be done in polynomial time.
\end{theorem}

\begin{proof}
    As in the proof of Theorem \ref{thm:BN_linear_top_k}, the computing a policy for each value of $\phi_{(\x, \z)}$, for $(\x, \z) \in \inter$, can be done efficiently if and only if, for a given strategy profile $\eta$, the integral of $h$ over the set 
    \begin{align*}
        U_{(\x_j, \z_j)} = \{(\x, \z) \in \inter: f(\x, \eta(\z)) \geq f(\x_j, \z_j) \},
    \end{align*}
    where $\eta$ can be though of as the strategy of an agent of the form $(\x, \z)$. Previously, in Theorem \ref{thm:BN_linear_top_k}, $\eta$ was the identity since all agents, expect potentially $\aj_j$ where assumed to be truthful. The key difference in the case of an $\epsilon$-dominant strategy equilibrium is that $U_{(\x_j, \z_j)}$ needs to account for any strategy profile $\eta$. That is $U_{(\x_j, \z_j)}$ should be the set of all possible agents such that there exists a map $\eta:I^s \rightarrow I^s$ with $f(\x, \eta(\z)) \geq f(\x_j, \z_j)$. 
    Since $f$ is linear, maximizing $f$ with respect to any dimension $d \in [s]$ can be achieved by simply taking $z_d = \min(I)$ if the $d^{\text{th}}$ coefficient is negative and $z_d = \max(I)$ if the $d^{\text{th}}$ is positive, let $z_d^*$ the maximizing value of the $d^{\text{th}}$ dimension. Let $\z^* = \langle z_1^*, ..., z_s^* \rangle$, then 
    \begin{align*}
        U_{(\x_j, \z_j)} = \{(\x, \z) \in \inter: f(\x, \z^*) \geq f(\x_j, \z_j)\}
    \end{align*}
    Since $\z^*$ can be computed in at most $s$ steps, the boundary conditions on $U_{(\x_j, \z_j)}$ can be computed efficiently. 
    Thus, using the exact techniques in the Bayes-Nash case, the term 
    \begin{align*}
        p_{U_{(\x_j, \z_j)}} = \int_{U_{(\x_j, \z_j)}}h(\x, \z) d\x d\z
    \end{align*}
    can be computed in polynomial time, which gives both the policy of WGHTAUDIT and the value of $\epsilon$.
\end{proof}


==> runningExample.tex <==
\section{Running Example}

\subsection{Top-$k$}
Suppose that agents are applying for need-based assistance for those at risk of homelessness. 
The principal has only a limited number of resources, say $k$, that are able to be distributed among the agents.
The top-$k$ scoring agents will be given assistance.


For simplicity, agents can be thought of as having four attributes: income, previous attempts to receive assistance, addiction, and mental-heath status.

Income exists on a continuous normalized spectrum $[0, 1]$. Previous attempt to receive assistance, addiction, and mental-health status are binary $\{0, 1\}$ which indicate existence.

\begin{figure}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         Attribute & Variable & Domain   & Type \\
        \hline \hline
         Income   & $x_1$ & $[0, 1]$ & Known \\
         \hline
         Previous Application & $x_2$ & $\{0, 1\}$ & Known \\
         \hline
         Addiction & $z_1$ & $\{0, 1\}$ & Self-Reported \\
         \hline 
         Mental Disorder & $z_2$ & $\{0, 1\}$ & Self-Reported\\
         \hline
    \end{tabular}
    \caption{Agent Attributes. Each agent is of the form $\aj = (x_1, x_2, z_1, z_2)$, where each type has uniform probability to exist.}
    
    \label{fig:attributes}
\end{figure}

Attributes of income and previous attempts to acquire assistance are considered to be know. Income can be verified with little effort from the principal by acquiring the tax return of applicants. Previous attempts to acquire aid can be verified by reaching out (email or phone call) to other agencies to determine if the applicant has made contact in the past. 

Addiction and mental-health status are self-reported attributes since they represent personal information that principal would not easily have access to and agents would be capable of misreporting. The values of these attributes are not entirely out of the principal's reach. For both attributes, addiction and mental-health status, the principal can, with some effort, verify the value of these attributes. For example, in the case of addiction, the principal could query the known associates of the agent to see if there is any report seeing the agent use drugs.

Suppose the principal wants a score function that considers a balance between the agents need for intervention, and how likely the intervention is to be successful. To achieve this balance, the principal could use a score function such as
\begin{align}
    f(x_1, x_2, z_1, z_2) = \frac{-x_1}{2} + x_2 - z_1 - z_2.
\end{align}

Then agents have an incentive to lie about not having addiction or mental health disorders. 

Suppose there are $n = 4$ agents competing for $k = 1$ resources with a budget of $B = 1$.
When the principal desires to find an audit policy which cause truthful reporting to be an $\epsilon$BNEQ with the lowest possible value of $\epsilon$, only agents reporting $z_1 = 0$ or $z_2 = 0$ will be audited. 
To find the optimal values of $\phi_{(\x, \z)}$, the principal needs to consider the difference that any agent reporting type $(\x, \z)$ has to gain. Since $\epsilon$ is the maximum value that \emph{any} agent can gain, the principal must consider the marginal expected gain of an agent reporting type $(\x, \z)$ and an agent reporting type $(\x, 1, 1)$.
If $T_{(\x, \z)}$ is the event that an agent of type $(\x, \z)$ is the top scoring agent and let $U_{(\x, \z)}$ the space of agents with scores greater than $(\x, \z)$, then the expected value of an agent of type $(\x, 1, 1)$ reporting type $(\x, \z)$ is
\begin{align*}
         & \mathbb{P}\big(T_{(\x, \z)}\big)(1 - \phi_{(\x, \z)}) - \mathbb{P}\big(T_{(\x, 1, 1)}\big) = \epsilon \\
    \iff & \phi_{(\x, \z)} = \frac{\mathbb{P}\big(T_{(\x, \z)}\big) - \mathbb{P}\big(T_{(\x, 1, 1)}\big) - \epsilon}{\mathbb{P}\big(T_{(\x, \z)}\big)} \\
    \iff & \phi_{(\x, \z)} = \frac{1 - 3|U_{(\x, \z)}| - 3|U_{(\x, \z)}|^2 - |U_{(\x, \z)}|^3  - 1  + 3|U_{(\x, 1, 1)}| + 3|U_{(\x, 1, 1)}|^2 + |U_{(\x, 1, 1)}|^3 - \epsilon}{1 - 3|U_{(\x, \z)}| - 3|U_{(\x, \z)}|^2 - |U_{(\x, \z)}|^3}\\
\end{align*}
Thus, for any agent reporting type $(\x, \z)$ the value of $\phi_{(\x, \z)}$ contains only a single unknown variable $\epsilon$, the depends of which is linear.

Therefore, for any realization of the $4$ agents $\{\aj_1, \aj_2, \aj_3, \aj_4\}$ the value of each $\phi_{\aj}$ can be derived by solving the equation

\begin{align*}
    \phi_{a_1} + \phi_{a_2} + \phi_{a_3} + \phi_{a_4} = 1
\end{align*}












